Analytical travelling vortex solutions of hyperbolic equations for validating very high order schemes

Testing the order of accuracy of (very) high order methods for shallow water (and Euler) equations is a delicate operation and the test cases are the crucial starting point of this operation. We provide a short derivation of vortex-like analytical solutions in 2 dimensions for the shallow water equations (and, hence, Euler equations) that can be used to test the order of accuracy of numerical methods. These solutions have different smoothness in their derivatives (up to $\mathcal C^\infty$) and can be used accordingly to the order of accuracy of the scheme to test.

==> data/SteadyVortex2/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   3.488e-04  &  0.000  &  2.280e-03 & 0.000  &  2.278e-03 & 0.000 \\ 
   16  &   8.466e-05  &  2.043  &  7.451e-04 & 1.613  &  7.451e-04 & 1.612 \\ 
   32  &   3.862e-05  &  1.132  &  1.119e-04 & 2.735  &  1.120e-04 & 2.734 \\ 
   64  &   2.285e-06  &  4.079  &  1.475e-05 & 2.924  &  1.475e-05 & 2.924 \\ 
  128  &   1.070e-07  &  4.417  &  1.072e-06 & 3.782  &  1.072e-06 & 3.782 \\ 
  256  &   4.349e-09  &  4.620  &  6.550e-08 & 4.033  &  6.550e-08 & 4.033 \\ 
  512  &   2.302e-10  &  4.240  &  3.851e-09 & 4.088  &  3.851e-09 & 4.088 \\ 


==> data/SteadyVortex3/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   3.330e-04  &  0.000  &  1.879e-03 & 0.000  &  1.880e-03 & 0.000 \\ 
   16  &   1.233e-04  &  1.434  &  8.613e-04 & 1.125  &  8.613e-04 & 1.126 \\ 
   32  &   4.730e-05  &  1.382  &  1.432e-04 & 2.588  &  1.432e-04 & 2.588 \\ 
   64  &   2.610e-06  &  4.180  &  1.546e-05 & 3.212  &  1.546e-05 & 3.211 \\ 
  128  &   9.876e-08  &  4.724  &  8.314e-07 & 4.217  &  8.315e-07 & 4.217 \\ 
  256  &   3.373e-09  &  4.872  &  3.030e-08 & 4.778  &  3.030e-08 & 4.778 \\ 
  512  &   1.354e-10  &  4.638  &  1.197e-09 & 4.662  &  1.197e-09 & 4.662 \\ 

==> data/SteadyVortex9/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   4.658e-04  &  0.000  &  2.475e-03 & 0.000  &  2.476e-03 & 0.000 \\ 
   16  &   2.286e-04  &  1.027  &  1.185e-03 & 1.063  &  1.185e-03 & 1.064 \\ 
   32  &   8.170e-05  &  1.484  &  3.710e-04 & 1.675  &  3.710e-04 & 1.675 \\ 
   64  &   1.516e-05  &  2.430  &  8.567e-05 & 2.114  &  8.568e-05 & 2.114 \\ 
  128  &   1.497e-06  &  3.340  &  1.177e-05 & 2.864  &  1.177e-05 & 2.864 \\ 
  256  &   6.913e-08  &  4.437  &  1.037e-06 & 3.504  &  1.037e-06 & 3.504 \\ 
  512  &   2.263e-09  &  4.933  &  3.900e-08 & 4.733  &  3.900e-08 & 4.733 \\ 


==> data/SteadyVortexCos/p1/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   5.878e-05  &  0.000  &  2.815e-04 & 0.000  &  2.816e-04 & 0.000 \\ 
   50  &   8.498e-06  &  2.790  &  6.062e-05 & 2.215  &  6.062e-05 & 2.216 \\ 
  100  &   1.080e-06  &  2.976  &  1.359e-05 & 2.157  &  1.359e-05 & 2.157 \\ 
  200  &   1.252e-07  &  3.108  &  2.829e-06 & 2.265  &  2.829e-06 & 2.264 \\ 
  300  &   3.483e-08  &  3.156  &  1.085e-06 & 2.364  &  1.085e-06 & 2.364 \\ 
  400  &   1.395e-08  &  3.182  &  5.430e-07 & 2.406  &  5.430e-07 & 2.406 \\ 
  500  &   6.848e-09  &  3.187  &  3.151e-07 & 2.439  &  3.151e-07 & 2.439 \\ 
  600  &   3.819e-09  &  3.202  &  2.013e-07 & 2.459  &  2.013e-07 & 2.459 \\ 


==> data/SteadyVortexCos/p1/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   3.592e-05  &  0.000  &  6.846e-04 & 0.000  &  6.846e-04 & 0.000 \\ 
   50  &   2.742e-06  &  3.711  &  1.387e-04 & 2.303  &  1.387e-04 & 2.303 \\ 
  100  &   2.951e-07  &  3.216  &  2.788e-05 & 2.315  &  2.788e-05 & 2.315 \\ 
  200  &   3.932e-08  &  2.908  &  5.260e-06 & 2.406  &  5.260e-06 & 2.406 \\ 
  300  &   1.259e-08  &  2.808  &  1.961e-06 & 2.434  &  1.961e-06 & 2.434 \\ 
  400  &   5.483e-09  &  2.890  &  9.716e-07 & 2.440  &  9.716e-07 & 2.440 \\ 
  500  &   2.854e-09  &  2.926  &  5.647e-07 & 2.432  &  5.647e-07 & 2.432 \\ 
  600  &   1.683e-09  &  2.895  &  3.628e-07 & 2.427  &  3.628e-07 & 2.427 \\ 


==> data/SteadyVortexCos/p2/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   5.780e-05  &  0.000  &  2.566e-04 & 0.000  &  2.565e-04 & 0.000 \\ 
   50  &   6.312e-06  &  3.195  &  3.094e-05 & 3.052  &  3.094e-05 & 3.051 \\ 
  100  &   3.260e-07  &  4.275  &  2.892e-06 & 3.420  &  2.892e-06 & 3.419 \\ 
  200  &   1.369e-08  &  4.573  &  1.786e-07 & 4.017  &  1.786e-07 & 4.017 \\ 
  300  &   2.122e-09  &  4.599  &  3.432e-08 & 4.067  &  3.432e-08 & 4.067 \\ 
  400  &   6.391e-10  &  4.171  &  1.061e-08 & 4.082  &  1.061e-08 & 4.081 \\ 
  500  &   3.087e-10  &  3.261  &  4.295e-09 & 4.052  &  4.293e-09 & 4.054 \\ 
  600  &   1.736e-10  &  3.156  &  2.065e-09 & 4.015  &  2.065e-09 & 4.014 \\ 


==> data/SteadyVortexCos/p2/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   5.884e-05  &  0.000  &  5.081e-04 & 0.000  &  5.082e-04 & 0.000 \\ 
   50  &   2.294e-06  &  4.681  &  5.198e-05 & 3.289  &  5.198e-05 & 3.289 \\ 
  100  &   8.318e-08  &  4.786  &  3.463e-06 & 3.908  &  3.463e-06 & 3.908 \\ 
  200  &   3.022e-09  &  4.783  &  2.069e-07 & 4.065  &  2.069e-07 & 4.065 \\ 
  300  &   5.125e-10  &  4.376  &  4.040e-08 & 4.028  &  4.040e-08 & 4.028 \\ 
  400  &   2.069e-10  &  3.153  &  1.277e-08 & 4.002  &  1.277e-08 & 4.002 \\ 
  500  &   1.206e-10  &  2.419  &  5.227e-09 & 4.005  &  5.225e-09 & 4.006 \\ 
  600  &   8.053e-11  &  2.214  &  2.512e-09 & 4.019  &  2.511e-09 & 4.018 \\ 


==> data/SteadyVortexCos/p3/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   5.103e-05  &  0.000  &  2.867e-04 & 0.000  &  2.869e-04 & 0.000 \\ 
   50  &   7.619e-06  &  2.744  &  3.328e-05 & 3.107  &  3.328e-05 & 3.108 \\ 
  100  &   3.272e-07  &  4.541  &  2.615e-06 & 3.670  &  2.615e-06 & 3.670 \\ 
  200  &   1.122e-08  &  4.867  &  9.849e-08 & 4.730  &  9.848e-08 & 4.731 \\ 
  300  &   1.557e-09  &  4.870  &  1.446e-08 & 4.732  &  1.446e-08 & 4.732 \\ 
  400  &   3.832e-10  &  4.873  &  3.772e-09 & 4.670  &  3.772e-09 & 4.670 \\ 
  500  &   1.522e-10  &  4.137  &  1.342e-09 & 4.631  &  1.342e-09 & 4.630 \\ 
  600  &   7.994e-11  &  3.533  &  5.772e-10 & 4.628  &  5.771e-10 & 4.630 \\ 


==> data/SteadyVortexCos/p3/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   9.827e-05  &  0.000  &  6.998e-04 & 0.000  &  7.001e-04 & 0.000 \\ 
   50  &   4.261e-06  &  4.527  &  5.686e-05 & 3.622  &  5.686e-05 & 3.622 \\ 
  100  &   1.549e-07  &  4.781  &  2.601e-06 & 4.450  &  2.601e-06 & 4.450 \\ 
  200  &   5.235e-09  &  4.887  &  9.659e-08 & 4.751  &  9.658e-08 & 4.751 \\ 
  300  &   7.430e-10  &  4.815  &  1.417e-08 & 4.734  &  1.417e-08 & 4.734 \\ 
  400  &   2.424e-10  &  3.893  &  3.609e-09 & 4.753  &  3.609e-09 & 4.753 \\ 
  500  &   1.322e-10  &  2.717  &  1.248e-09 & 4.760  &  1.247e-09 & 4.760 \\ 
  600  &   8.976e-11  &  2.124  &  5.250e-10 & 4.747  &  5.250e-10 & 4.747 \\ 


==> data/SteadyVortexExp/p2/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   4.895e-04  &  0.000  &  3.614e-03 & 0.000  &  3.613e-03 & 0.000 \\ 
   16  &   3.576e-04  &  0.453  &  1.962e-03 & 0.881  &  1.962e-03 & 0.881 \\ 
   32  &   1.362e-04  &  1.393  &  7.817e-04 & 1.328  &  7.815e-04 & 1.328 \\ 
   64  &   3.040e-05  &  2.163  &  2.167e-04 & 1.851  &  2.168e-04 & 1.850 \\ 
  128  &   3.640e-06  &  3.062  &  4.345e-05 & 2.319  &  4.345e-05 & 2.319 \\ 
  256  &   2.714e-07  &  3.745  &  4.926e-06 & 3.141  &  4.926e-06 & 3.141 \\ 
  512  &   1.088e-08  &  4.641  &  3.517e-07 & 3.808  &  3.517e-07 & 3.808 \\ 
% 1024  &   4.269e-10  &  4.672  &  1.350e-08 & 4.703  &  1.350e-08 & 4.703 \\ 


==> data/SteadyVortexExp/p2/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   1.761e-04  &  0.000  &  1.061e-03 & 0.000  &  1.061e-03 & 0.000 \\ 
   50  &   5.484e-05  &  1.683  &  3.591e-04 & 1.563  &  3.591e-04 & 1.563 \\ 
  100  &   7.919e-06  &  2.792  &  8.049e-05 & 2.157  &  8.049e-05 & 2.157 \\ 
  200  &   7.454e-07  &  3.409  &  1.127e-05 & 2.836  &  1.127e-05 & 2.836 \\ 
  300  &   1.352e-07  &  4.211  &  2.918e-06 & 3.333  &  2.918e-06 & 3.333 \\ 
  400  &   3.547e-08  &  4.651  &  1.019e-06 & 3.657  &  1.019e-06 & 3.657 \\ 
  500  &   1.219e-08  &  4.786  &  3.905e-07 & 4.298  &  3.905e-07 & 4.298 \\ 
  600  &   5.072e-09  &  4.809  &  1.677e-07 & 4.638  &  1.677e-07 & 4.637 \\ 


==> data/SteadyVortexExp/p2/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   2.910e-04  &  0.000  &  3.486e-03 & 0.000  &  3.485e-03 & 0.000 \\ 
   50  &   6.799e-05  &  2.098  &  9.009e-04 & 1.952  &  9.009e-04 & 1.952 \\ 
  100  &   6.188e-06  &  3.458  &  1.574e-04 & 2.517  &  1.574e-04 & 2.517 \\ 
  200  &   2.535e-07  &  4.610  &  1.549e-05 & 3.345  &  1.549e-05 & 3.345 \\ 
  300  &   3.018e-08  &  5.248  &  3.922e-06 & 3.387  &  3.922e-06 & 3.387 \\ 
  400  &   6.926e-09  &  5.117  &  1.208e-06 & 4.094  &  1.208e-06 & 4.094 \\ 
  500  &   2.305e-09  &  4.931  &  4.499e-07 & 4.425  &  4.499e-07 & 4.425 \\ 
  600  &   9.590e-10  &  4.810  &  2.010e-07 & 4.420  &  2.010e-07 & 4.420 \\ 


==> data/SteadyVortexExp/p3/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   3.841e-04  &  0.000  &  3.156e-03 & 0.000  &  3.155e-03 & 0.000 \\ 
   16  &   1.891e-04  &  1.022  &  1.562e-03 & 1.015  &  1.562e-03 & 1.014 \\ 
   32  &   1.153e-04  &  0.714  &  6.171e-04 & 1.340  &  6.171e-04 & 1.340 \\ 
   64  &   2.549e-05  &  2.177  &  1.616e-04 & 1.933  &  1.616e-04 & 1.933 \\ 
  128  &   2.782e-06  &  3.196  &  2.710e-05 & 2.576  &  2.710e-05 & 2.576 \\ 
  256  &   1.619e-07  &  4.103  &  2.733e-06 & 3.310  &  2.733e-06 & 3.310 \\ 
  512  &   5.609e-09  &  4.851  &  1.352e-07 & 4.337  &  1.352e-07 & 4.337 \\ 
% 1024  &   2.375e-10  &  4.562  &  5.587e-09 & 4.597  &  5.587e-09 & 4.597 \\ 


==> data/SteadyVortexExp/p3/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   1.617e-04  &  0.000  &  8.465e-04 & 0.000  &  8.465e-04 & 0.000 \\ 
   50  &   4.767e-05  &  1.762  &  2.751e-04 & 1.621  &  2.751e-04 & 1.622 \\ 
  100  &   6.389e-06  &  2.899  &  5.407e-05 & 2.347  &  5.407e-05 & 2.347 \\ 
  200  &   4.886e-07  &  3.709  &  6.269e-06 & 3.109  &  6.269e-06 & 3.109 \\ 
  300  &   7.643e-08  &  4.575  &  1.521e-06 & 3.493  &  1.521e-06 & 3.493 \\ 
  400  &   1.877e-08  &  4.881  &  4.379e-07 & 4.328  &  4.379e-07 & 4.328 \\ 
  500  &   6.295e-09  &  4.896  &  1.516e-07 & 4.754  &  1.516e-07 & 4.754 \\ 
  600  &   2.624e-09  &  4.800  &  6.320e-08 & 4.799  &  6.320e-08 & 4.799 \\ 


==> data/SteadyVortexExp/p3/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   2.694e-04  &  0.000  &  2.848e-03 & 0.000  &  2.848e-03 & 0.000 \\ 
   50  &   5.684e-05  &  2.245  &  6.747e-04 & 2.077  &  6.746e-04 & 2.078 \\ 
  100  &   4.179e-06  &  3.766  &  9.516e-05 & 2.826  &  9.516e-05 & 2.826 \\ 
  200  &   1.372e-07  &  4.929  &  8.798e-06 & 3.435  &  8.798e-06 & 3.435 \\ 
  300  &   1.737e-08  &  5.098  &  1.793e-06 & 3.924  &  1.793e-06 & 3.924 \\ 
  400  &   4.236e-09  &  4.904  &  4.952e-07 & 4.472  &  4.952e-07 & 4.472 \\ 
  500  &   1.451e-09  &  4.802  &  1.815e-07 & 4.497  &  1.815e-07 & 4.497 \\ 
  600  &   6.103e-10  &  4.749  &  7.889e-08 & 4.571  &  7.889e-08 & 4.571 \\ 


==> data/SteadyVortexExp/p4/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   4.365e-04  &  0.000  &  2.883e-03 & 0.000  &  2.894e-03 & 0.000 \\ 
   16  &   2.912e-04  &  0.584  &  1.293e-03 & 1.157  &  1.293e-03 & 1.163 \\ 
   32  &   1.155e-04  &  1.334  &  5.657e-04 & 1.192  &  5.657e-04 & 1.192 \\ 
   64  &   2.539e-05  &  2.186  &  1.472e-04 & 1.942  &  1.472e-04 & 1.942 \\ 
  128  &   2.680e-06  &  3.244  &  2.315e-05 & 2.669  &  2.315e-05 & 2.669 \\ 
  256  &   1.448e-07  &  4.209  &  2.272e-06 & 3.349  &  2.272e-06 & 3.349 \\ 
  512  &   4.797e-09  &  4.916  &  1.017e-07 & 4.481  &  1.017e-07 & 4.481 \\ 
% 1024  &   2.088e-10  &  4.522  &  4.339e-09 & 4.552  &  4.339e-09 & 4.551 \\ 


==> data/SteadyVortexExp/p4/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   1.270e-04  &  0.000  &  7.922e-04 & 0.000  &  7.922e-04 & 0.000 \\ 
   50  &   4.701e-05  &  1.434  &  2.509e-04 & 1.659  &  2.509e-04 & 1.659 \\ 
  100  &   6.253e-06  &  2.910  &  4.716e-05 & 2.412  &  4.716e-05 & 2.412 \\ 
  200  &   4.492e-07  &  3.799  &  5.254e-06 & 3.166  &  5.254e-06 & 3.166 \\ 
  300  &   6.748e-08  &  4.675  &  1.223e-06 & 3.595  &  1.223e-06 & 3.595 \\ 
  400  &   1.624e-08  &  4.952  &  3.336e-07 & 4.516  &  3.336e-07 & 4.516 \\ 
  500  &   5.387e-09  &  4.944  &  1.142e-07 & 4.805  &  1.142e-07 & 4.805 \\ 
  600  &   2.245e-09  &  4.801  &  4.765e-08 & 4.793  &  4.765e-08 & 4.793 \\ 


==> data/SteadyVortexExp/p4/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   2.514e-04  &  0.000  &  2.619e-03 & 0.000  &  2.619e-03 & 0.000 \\ 
   50  &   5.631e-05  &  2.158  &  6.180e-04 & 2.083  &  6.180e-04 & 2.083 \\ 
  100  &   4.048e-06  &  3.798  &  8.056e-05 & 2.939  &  8.056e-05 & 2.939 \\ 
  200  &   1.288e-07  &  4.974  &  7.346e-06 & 3.455  &  7.346e-06 & 3.455 \\ 
  300  &   1.669e-08  &  5.039  &  1.395e-06 & 4.097  &  1.395e-06 & 4.097 \\ 
  400  &   4.113e-09  &  4.870  &  3.827e-07 & 4.496  &  3.827e-07 & 4.496 \\ 
  500  &   1.408e-09  &  4.802  &  1.395e-07 & 4.523  &  1.395e-07 & 4.523 \\ 
  600  &   5.893e-10  &  4.778  &  6.044e-08 & 4.587  &  6.044e-08 & 4.587 \\ 


==> data/SteadyVortexExp/p5/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   4.607e-04  &  0.000  &  2.728e-03 & 0.000  &  2.733e-03 & 0.000 \\ 
   16  &   2.974e-04  &  0.632  &  1.350e-03 & 1.015  &  1.350e-03 & 1.018 \\ 
   32  &   9.707e-05  &  1.615  &  5.199e-04 & 1.376  &  5.198e-04 & 1.377 \\ 
   64  &   2.584e-05  &  1.909  &  1.429e-04 & 1.864  &  1.428e-04 & 1.863 \\ 
  128  &   2.784e-06  &  3.214  &  2.212e-05 & 2.691  &  2.212e-05 & 2.691 \\ 
  256  &   1.494e-07  &  4.220  &  2.157e-06 & 3.358  &  2.157e-06 & 3.358 \\ 
  512  &   4.865e-09  &  4.940  &  9.604e-08 & 4.489  &  9.604e-08 & 4.489 \\ 
% 1024  &   2.073e-10  &  4.553  &  4.132e-09 & 4.539  &  4.132e-09 & 4.539 \\ 


==> data/SteadyVortexExp/p5/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   1.253e-04  &  0.000  &  7.971e-04 & 0.000  &  7.972e-04 & 0.000 \\ 
   50  &   4.601e-05  &  1.445  &  2.424e-04 & 1.717  &  2.425e-04 & 1.717 \\ 
  100  &   6.604e-06  &  2.800  &  4.518e-05 & 2.424  &  4.518e-05 & 2.424 \\ 
  200  &   4.652e-07  &  3.828  &  4.995e-06 & 3.177  &  4.995e-06 & 3.177 \\ 
  300  &   6.935e-08  &  4.694  &  1.165e-06 & 3.590  &  1.165e-06 & 3.590 \\ 
  400  &   1.657e-08  &  4.976  &  3.157e-07 & 4.538  &  3.157e-07 & 4.538 \\ 
  500  &   5.466e-09  &  4.970  &  1.076e-07 & 4.823  &  1.076e-07 & 4.823 \\ 
  600  &   2.263e-09  &  4.836  &  4.520e-08 & 4.759  &  4.520e-08 & 4.759 \\ 


==> data/SteadyVortexExp/p5/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   2.532e-04  &  0.000  &  2.491e-03 & 0.000  &  2.490e-03 & 0.000 \\ 
   50  &   5.783e-05  &  2.130  &  6.108e-04 & 2.028  &  6.108e-04 & 2.028 \\ 
  100  &   4.365e-06  &  3.728  &  7.752e-05 & 2.978  &  7.752e-05 & 2.978 \\ 
  200  &   1.422e-07  &  4.940  &  7.032e-06 & 3.463  &  7.032e-06 & 3.463 \\ 
  300  &   1.852e-08  &  5.026  &  1.328e-06 & 4.111  &  1.328e-06 & 4.111 \\ 
  400  &   4.567e-09  &  4.867  &  3.636e-07 & 4.503  &  3.636e-07 & 4.503 \\ 
  500  &   1.568e-09  &  4.790  &  1.325e-07 & 4.525  &  1.325e-07 & 4.525 \\ 
  600  &   6.573e-10  &  4.770  &  5.732e-08 & 4.595  &  5.732e-08 & 4.595 \\ 


==> data/SteadyVortexTan/p2/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   4.814e-04  &  0.000  &  3.607e-03 & 0.000  &  3.607e-03 & 0.000 \\ 
   16  &   3.568e-04  &  0.432  &  1.934e-03 & 0.900  &  1.934e-03 & 0.899 \\ 
   32  &   1.337e-04  &  1.416  &  7.667e-04 & 1.334  &  7.666e-04 & 1.335 \\ 
   64  &   2.969e-05  &  2.170  &  2.128e-04 & 1.849  &  2.128e-04 & 1.849 \\ 
  128  &   3.571e-06  &  3.056  &  4.262e-05 & 2.320  &  4.263e-05 & 2.320 \\ 
  256  &   2.662e-07  &  3.746  &  4.832e-06 & 3.141  &  4.832e-06 & 3.141 \\ 
  512  &   1.067e-08  &  4.641  &  3.444e-07 & 3.811  &  3.444e-07 & 3.810 \\ 
% 1024  &   4.185e-10  &  4.672  &  1.321e-08 & 4.704  &  1.321e-08 & 4.704 \\ 


==> data/SteadyVortexTan/p2/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   1.757e-04  &  0.000  &  1.041e-03 & 0.000  &  1.041e-03 & 0.000 \\ 
   50  &   5.372e-05  &  1.710  &  3.521e-04 & 1.564  &  3.521e-04 & 1.564 \\ 
  100  &   7.757e-06  &  2.792  &  7.912e-05 & 2.154  &  7.913e-05 & 2.154 \\ 
  200  &   7.309e-07  &  3.408  &  1.105e-05 & 2.840  &  1.105e-05 & 2.840 \\ 
  300  &   1.326e-07  &  4.210  &  2.862e-06 & 3.332  &  2.862e-06 & 3.332 \\ 
  400  &   3.478e-08  &  4.651  &  9.987e-07 & 3.660  &  9.987e-07 & 3.660 \\ 
  500  &   1.195e-08  &  4.786  &  3.824e-07 & 4.302  &  3.824e-07 & 4.302 \\ 
  600  &   4.975e-09  &  4.808  &  1.641e-07 & 4.639  &  1.641e-07 & 4.639 \\ 


==> data/SteadyVortexTan/p2/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   2.845e-04  &  0.000  &  3.417e-03 & 0.000  &  3.417e-03 & 0.000 \\ 
   50  &   6.571e-05  &  2.114  &  8.826e-04 & 1.953  &  8.826e-04 & 1.953 \\ 
  100  &   5.972e-06  &  3.460  &  1.543e-04 & 2.516  &  1.543e-04 & 2.516 \\ 
  200  &   2.443e-07  &  4.612  &  1.519e-05 & 3.345  &  1.519e-05 & 3.345 \\ 
  300  &   2.916e-08  &  5.242  &  3.844e-06 & 3.389  &  3.844e-06 & 3.389 \\ 
  400  &   6.695e-09  &  5.115  &  1.182e-06 & 4.098  &  1.183e-06 & 4.098 \\ 
  500  &   2.229e-09  &  4.928  &  4.405e-07 & 4.426  &  4.405e-07 & 4.426 \\ 
  600  &   9.280e-10  &  4.807  &  1.968e-07 & 4.419  &  1.968e-07 & 4.419 \\ 


==> data/SteadyVortexTan/p3/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   3.561e-04  &  0.000  &  3.010e-03 & 0.000  &  3.005e-03 & 0.000 \\ 
   16  &   1.725e-04  &  1.046  &  1.323e-03 & 1.186  &  1.323e-03 & 1.184 \\ 
   32  &   1.016e-04  &  0.763  &  5.062e-04 & 1.386  &  5.061e-04 & 1.386 \\ 
   64  &   1.930e-05  &  2.397  &  1.231e-04 & 2.040  &  1.231e-04 & 2.040 \\ 
  128  &   2.056e-06  &  3.231  &  1.942e-05 & 2.665  &  1.942e-05 & 2.665 \\ 
  256  &   1.113e-07  &  4.208  &  1.904e-06 & 3.350  &  1.904e-06 & 3.350 \\ 
  512  &   3.814e-09  &  4.867  &  8.508e-08 & 4.484  &  8.508e-08 & 4.484 \\ 
% 1024  &   1.702e-10  &  4.486  &  3.547e-09 & 4.584  &  3.547e-09 & 4.584 \\ 


==> data/SteadyVortexTan/p3/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   1.390e-04  &  0.000  &  6.769e-04 & 0.000  &  6.769e-04 & 0.000 \\ 
   50  &   3.709e-05  &  1.906  &  2.113e-04 & 1.680  &  2.113e-04 & 1.680 \\ 
  100  &   4.787e-06  &  2.954  &  3.986e-05 & 2.406  &  3.986e-05 & 2.406 \\ 
  200  &   3.431e-07  &  3.802  &  4.450e-06 & 3.163  &  4.449e-06 & 3.163 \\ 
  300  &   5.208e-08  &  4.649  &  1.019e-06 & 3.635  &  1.019e-06 & 3.635 \\ 
  400  &   1.270e-08  &  4.906  &  2.785e-07 & 4.510  &  2.785e-07 & 4.510 \\ 
  500  &   4.280e-09  &  4.874  &  9.539e-08 & 4.801  &  9.539e-08 & 4.801 \\ 
  600  &   1.799e-09  &  4.754  &  3.953e-08 & 4.832  &  3.953e-08 & 4.832 \\ 


==> data/SteadyVortexTan/p3/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   2.082e-04  &  0.000  &  2.342e-03 & 0.000  &  2.342e-03 & 0.000 \\ 
   50  &   3.734e-05  &  2.479  &  4.981e-04 & 2.233  &  4.981e-04 & 2.233 \\ 
  100  &   2.478e-06  &  3.913  &  6.612e-05 & 2.913  &  6.612e-05 & 2.913 \\ 
  200  &   7.905e-08  &  4.970  &  6.137e-06 & 3.429  &  6.137e-06 & 3.429 \\ 
  300  &   1.027e-08  &  5.035  &  1.148e-06 & 4.134  &  1.148e-06 & 4.134 \\ 
  400  &   2.548e-09  &  4.843  &  3.160e-07 & 4.484  &  3.160e-07 & 4.484 \\ 
  500  &   8.843e-10  &  4.743  &  1.152e-07 & 4.522  &  1.152e-07 & 4.522 \\ 
  600  &   3.766e-10  &  4.682  &  4.993e-08 & 4.585  &  4.994e-08 & 4.585 \\ 


==> data/SteadyVortexTan/p4/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\
    8  &   4.239e-04  &  0.000  &  2.598e-03 & 0.000  &  2.603e-03 & 0.000 \\ 
   16  &   2.296e-04  &  0.885  &  1.183e-03 & 1.135  &  1.183e-03 & 1.137 \\ 
   32  &   8.181e-05  &  1.489  &  3.711e-04 & 1.673  &  3.712e-04 & 1.673 \\ 
   64  &   1.514e-05  &  2.434  &  8.567e-05 & 2.115  &  8.567e-05 & 2.115 \\ 
  128  &   1.496e-06  &  3.339  &  1.177e-05 & 2.864  &  1.177e-05 & 2.864 \\ 
  256  &   6.900e-08  &  4.439  &  1.037e-06 & 3.504  &  1.037e-06 & 3.504 \\ 
  512  &   2.269e-09  &  4.927  &  3.899e-08 & 4.733  &  3.899e-08 & 4.733 \\ 
% 1024  &   1.110e-10  &  4.354  &  1.713e-09 & 4.509  &  1.713e-09 & 4.509 \\ 


==> data/SteadyVortexTan/p4/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   1.036e-04  &  0.000  &  6.414e-04 & 0.000  &  6.414e-04 & 0.000 \\ 
   50  &   3.006e-05  &  1.785  &  1.562e-04 & 2.038  &  1.562e-04 & 2.038 \\ 
  100  &   3.667e-06  &  3.035  &  2.535e-05 & 2.623  &  2.535e-05 & 2.623 \\ 
  200  &   2.231e-07  &  4.039  &  2.677e-06 & 3.243  &  2.677e-06 & 3.243 \\ 
  300  &   3.161e-08  &  4.819  &  5.140e-07 & 4.070  &  5.140e-07 & 4.070 \\ 
  400  &   7.546e-09  &  4.979  &  1.296e-07 & 4.788  &  1.296e-07 & 4.788 \\ 
  500  &   2.539e-09  &  4.881  &  4.372e-08 & 4.871  &  4.372e-08 & 4.871 \\ 
  600  &   1.088e-09  &  4.648  &  1.872e-08 & 4.653  &  1.872e-08 & 4.653 \\ 


==> data/SteadyVortexTan/p4/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   1.703e-04  &  0.000  &  1.842e-03 & 0.000  &  1.842e-03 & 0.000 \\ 
   50  &   2.681e-05  &  2.668  &  3.516e-04 & 2.390  &  3.516e-04 & 2.390 \\ 
  100  &   1.547e-06  &  4.115  &  3.938e-05 & 3.158  &  3.938e-05 & 3.158 \\ 
  200  &   4.826e-08  &  5.002  &  3.383e-06 & 3.541  &  3.383e-06 & 3.541 \\ 
  300  &   6.510e-09  &  4.940  &  5.590e-07 & 4.440  &  5.590e-07 & 4.440 \\ 
  400  &   1.650e-09  &  4.771  &  1.528e-07 & 4.507  &  1.528e-07 & 4.507 \\ 
  500  &   5.810e-10  &  4.678  &  5.528e-08 & 4.557  &  5.528e-08 & 4.557 \\ 
  600  &   2.567e-10  &  4.480  &  2.382e-08 & 4.618  &  2.382e-08 & 4.619 \\ 


==> data/SteadyVortexTan/p5/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   3.706e-04  &  0.000  &  2.155e-03 & 0.000  &  2.157e-03 & 0.000 \\ 
   16  &   1.920e-04  &  0.948  &  1.132e-03 & 0.929  &  1.131e-03 & 0.931 \\ 
   32  &   7.159e-05  &  1.424  &  3.530e-04 & 1.681  &  3.530e-04 & 1.681 \\ 
   64  &   1.307e-05  &  2.454  &  6.902e-05 & 2.355  &  6.902e-05 & 2.355 \\ 
  128  &   1.220e-06  &  3.421  &  8.452e-06 & 3.030  &  8.452e-06 & 3.030 \\ 
  256  &   5.170e-08  &  4.560  &  6.688e-07 & 3.660  &  6.688e-07 & 3.660 \\ 
  512  &   1.695e-09  &  4.931  &  2.400e-08 & 4.800  &  2.400e-08 & 4.800 \\ 
% 1024  &   8.377e-11  &  4.338  &  1.056e-09 & 4.506  &  1.056e-09 & 4.506 \\ 


==> data/SteadyVortexTan/p5/convergence2.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   8.918e-05  &  0.000  &  5.002e-04 & 0.000  &  5.000e-04 & 0.000 \\ 
   50  &   2.638e-05  &  1.758  &  1.277e-04 & 1.970  &  1.277e-04 & 1.969 \\ 
  100  &   3.106e-06  &  3.086  &  1.880e-05 & 2.764  &  1.880e-05 & 2.764 \\ 
  200  &   1.713e-07  &  4.181  &  1.859e-06 & 3.338  &  1.859e-06 & 3.338 \\ 
  300  &   2.344e-08  &  4.905  &  3.186e-07 & 4.350  &  3.186e-07 & 4.350 \\ 
  400  &   5.577e-09  &  4.992  &  7.846e-08 & 4.872  &  7.846e-08 & 4.871 \\ 
  500  &   1.893e-09  &  4.841  &  2.675e-08 & 4.821  &  2.676e-08 & 4.821 \\ 
  600  &   8.167e-10  &  4.612  &  1.186e-08 & 4.460  &  1.186e-08 & 4.460 \\ 


==> data/SteadyVortexTan/p5/convergence4.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
   25  &   1.692e-04  &  0.000  &  1.669e-03 & 0.000  &  1.668e-03 & 0.000 \\ 
   50  &   2.290e-05  &  2.885  &  2.809e-04 & 2.571  &  2.808e-04 & 2.571 \\ 
  100  &   1.218e-06  &  4.233  &  2.758e-05 & 3.348  &  2.758e-05 & 3.348 \\ 
  200  &   3.909e-08  &  4.962  &  2.197e-06 & 3.650  &  2.197e-06 & 3.650 \\ 
  300  &   5.426e-09  &  4.870  &  3.519e-07 & 4.517  &  3.519e-07 & 4.517 \\ 
  400  &   1.396e-09  &  4.720  &  9.558e-08 & 4.531  &  9.559e-08 & 4.530 \\ 
  500  &   5.033e-10  &  4.571  &  3.436e-08 & 4.584  &  3.436e-08 & 4.585 \\ 
  600  &   2.290e-10  &  4.318  &  1.473e-08 & 4.647  &  1.473e-08 & 4.647 \\ 


==> data/SteadyVortexTan/p9/convergence.tex <==
  N   & Error h  &  Order h & Error u  &  Order u & Error v  &  Order v \\ 
    8  &   1.150e-04  &  0.000  &  6.678e-04 & 0.000  &  6.679e-04 & 0.000 \\ 
   16  &   6.887e-05  &  0.740  &  6.154e-04 & 0.118  &  6.147e-04 & 0.120 \\ 
   32  &   4.361e-05  &  0.659  &  3.393e-04 & 0.859  &  3.392e-04 & 0.858 \\ 
   64  &   1.468e-05  &  1.571  &  7.715e-05 & 2.137  &  7.712e-05 & 2.137 \\ 
  128  &   1.232e-06  &  3.575  &  7.141e-06 & 3.433  &  7.143e-06 & 3.432 \\ 
  256  &   4.670e-08  &  4.721  &  4.838e-07 & 3.884  &  4.838e-07 & 3.884 \\ 
  512  &   1.646e-09  &  4.826  &  1.756e-08 & 4.784  &  1.756e-08 & 4.784 \\ 
 1024  &   NaN  &  NaN  &  NaN & NaN  &  NaN & NaN \\ 

